Qiskit Pulse: Programming Quantum Computers Through the Cloud with Pulses

The quantum circuit model is an abstraction that hides the underlying physical implementation of gates and measurements on a quantum computer. For precise control of real quantum hardware, the ability to execute pulse and readout-level instructions is required. To that end, we introduce Qiskit Pulse, a pulse-level programming paradigm implemented as a module within Qiskit-Terra \cite{Qiskit}. To demonstrate the capabilities of Qiskit Pulse, we calibrate both un-echoed and echoed variants of the cross-resonance entangling gate with a pair of qubits on an IBM Quantum system accessible through the cloud. We perform Hamiltonian characterization of both single and two-pulse variants of the cross-resonance entangling gate with varying amplitudes on a cloud-based IBM Quantum system. We then transform these calibrated sequences into a high-fidelity CNOT gate by applying pre and post local-rotations to the qubits, achieving average gate fidelities of $F=0.981$ and $F=0.979$ for the un-echoed and echoed respectively. This is comparable to the standard backend CNOT fidelity of $F_{CX}=0.984$. Furthermore, to illustrate how users can access their results at different levels of the readout chain, we build a custom discriminator to investigate qubit readout correlations. Qiskit Pulse allows users to explore advanced control schemes such as optimal control theory, dynamical decoupling, and error mitigation that are not available within the circuit model.

==> pulse_model.tex <==
\section{Virtual Pulse ISA}
The pulse V-ISA is intended to be included as a coprocessor within an encompassing classical V-ISA which enables program control flow. We do not focus on including classical control flow within this work. Each sequence of pulse instructions in OpenPulse would be considered as a basic-pulse-block within an encompassing control-flow enabled V-ISA.

The instructions of the V-ISA are scheduled on \textit{channels} which execute in parallel and consume instructions from a FIFO queue. We follow an instruction \textit{allocation} and \textit{trigger} timing model which allows instructions to be absolutely scheduled in time. We provide synchronization instructions that guarantee that channels following the fence start with a flushed buffer, effectively resetting the local time of the pulse-block to $t=0$.

Every channel supports a \texttt{delay} instruction. All other instructions must either explicitly, or implicitly define a fixed, deterministic duration. This allows instructions within a basic pulse-block to be relatively scheduled in time across channels.

The fundamental stimulus channel of the V-ISA is the \texttt{pulse-channel} which is a subtype of \texttt{channel} and is mapped to a waveform stimulus channel in the quantum system. Each pulse-channel maintains a sideband modulation frequency, $f$ and a \textit{frame}, $\phi$ which tracks the phase of the output sideband and enables the implementation of \textit{virtual} Z-gates \cite{Mckay2017}. Pulse waveforms are output with the form $D_j =  \textrm{Re}\left[e^{i 2\pi f j dt + \phi}d_j \right]$, where $d_j$ is the jth output complex pulse sample. Pulse channels are typically indexed within hardware from [0, n-1] and are typically aliased as $\{d0, \ldots, d_{n_{q}-1}, m0, \ldots, m_{n_{q}-1}, u0, \ldots, u_{n_{u}-1}\}$, where $d$<i> and $m$<i> drive and measurement stimulus channels for one of the respectively indexed $n_q$ qubits and $u$<i> are one of the $n_u$ arbitrary control channels for the system. Pulse channels within the V-ISA are tied during compilation to target hardware channels through constraints. It is important to note that current-day qubits either have highly variable physical properties or stimulus channels and as a consequence permuting which pulse-channels belong to which qubits in a program will not give an equivalent result when run. As a consequence pulses must be engineered for their respective qubits.

Pulse channels support addressing instructions to allocate and load a pulse with a complex waveform. Pulse channels also augment the classical instruction set with instructions that support playing pulses and shifting the channel frame and frequency.

Acquisition instructions measure the qubit's state by sampling the output of a measurement stimulus pulse and are scheduled on acquisition channels. They must be arranged to align with corresponding measurement stimulus instructions to properly measure the respective qubit. Each acquire channel is constrained to a physical measurement chain in the hardware which typically includes ADC data acquisition, filtering, kerneling, and state discrimination. An acquisition channel outputs an unsigned integer value \texttt{iN}, but typically this will be a single bit (\texttt{i1}) for the standard qubit. Note that it may be possible that a given measurement stimulus measures multiple qubits in which case multiple acquisition instructions must be appropriately scheduled for the set of measured qubits.

This set of operations should have sufficient generality to program an arbitrary quantum computing system in the time-domain and be embedded within a larger V-ISA that might include both classical control flow and a traditional circuit-level description of a quantum program implemented as callable functions containing pulse operations. The benefit of the V-ISA is that a single software stack may provide the frontend for the rapidly developing homogeneous and heterogeneous hardware platforms within the quantum computing industry.

